Hypergraph Connectivity Augmentation in Strongly Polynomial Time

We consider hypergraph network design problems where the goal is to construct a hypergraph that satisfies certain connectivity requirements. For graph network design problems where the goal is to construct a graph that satisfies certain connectivity requirements, the number of edges in every feasible solution is at most quadratic in the number of vertices. In contrast, for hypergraph network design problems, we might have feasible solutions in which the number of hyperedges is exponential in the number of vertices. This presents an additional technical challenge in hypergraph network design problems compared to graph network design problems: in order to solve the problem in polynomial time, we first need to show that there exists a feasible solution in which the number of hyperedges is polynomial in the input size. The central theme of this work is to show that certain hypergraph network design problems admit solutions in which the number of hyperedges is polynomial in the number of vertices and moreover, can be solved in strongly polynomial time. Our work improves on the previous fastest pseudo-polynomial run-time for these problems. In addition, we develop strongly polynomial time algorithms that return near-uniform hypergraphs as solutions (i.e., every pair of hyperedges differ in size by at most one). As applications of our results, we derive the first strongly polynomial time algorithms for (i) degree-specified hypergraph connectivity augmentation using hyperedges, (ii) degree-specified hypergraph node-to-area connectivity augmentation using hyperedges, and (iii) degree-constrained mixed-hypergraph connectivity augmentation using hyperedges.

==> hypergraph-connectivity-augmentation-1.tex <==

\subsection{Hypergraph local connectivity augmentation using hyperedges}\label{sec:local-connectivity-augmentation-of-hypergraphs-using-hyperedges}
Graph local connectivity augmentation  using edges of minimum total weight problem is a classic network design problem that admits strongly polynomial-time algorithms %\cite{WN87, CS89, Fra92, nagamochi_ibaraki_2008_book, Frank-book}
\cite{WN87, CS89, Fra94, Fra92, Gab94, BHTP03, NGM97, BK00, LY13, CLP22-soda, CLP22-stoc, CHLP23}. 
Szigeti \cite{Szi99} proposed and studied a natural generalization to hypergraphs. The hypergraph local connectivity augmentation using hyperedges of minimum total weighted size 
%problem. Local connectivity augmentation of hypergraphs using hyperedges of minimum total weighted size is the following 
problem is the following: 
the input is a hypergraph $(G=(V, E), c: E\rightarrow \Z_+)$ and a target connectivity function $r: \binom{V}{2}\rightarrow \Z_{\ge 0}$. 
The goal is to find a hypergraph $(H=(V, E_H), w: E_H\rightarrow \Z_+)$ 
with minimum $\sum_{e\in E_H}|e|w(e)$ (i.e., minimum total weighted size), 
such that $\lambda_{(G+H, c+w)}(u, v)\ge r(\{u, v\})$ for every $u, v\in V$. 
\iffalse
where 
$(G_{c+w}=(V, E_{c+w}), c+w)$ is the hypergraph on vertex set $V$ and hyperedge set $E_{c+w}\coloneqq E\cup E_H$ with the weight of every hyperedge $e\in E_{c+w}$ being $c(e) + w(e)$ if $e\in E\cap E_H$ and $w(e)$ if $e\in E_H-E$, and $\lambda_{(G_{c+w}, c+w)}(u, v)$ is the value of a minimum $\{u, v\}$-cut in the hypergraph $(G_{c+w}, c+w)$. 
\fi
Szigeti \cite{Szi99} gave a min-max relation for this problem. 
Bern\'{a}th and Kir\'{a}ly \cite{Bernath-Kiraly} showed that there exists an optimal solution for this problem that is near-uniform. 
Our results imply that this problem can be solved in strongly polynomial time. 
\begin{theorem}\label{thm:local-connectivity-augmentation}
    Hypergraph local connectivity augmentation using hyperedges of minimum total weighted size problem can be solved in strongly polynomial time. 
    In particular, there exists a strongly polynomial-time algorithm to return an optimum solution $(H, w)$ such that $H$ is near-uniform and has $O(|V|)$ hyperedges, where $V$ is the vertex set of the input instance. 
    %Moreover, if the input instance also satisfies the condition that $m(V)/K_p\in \Z$ \knote{What is $m$? Need to fix this statement.}, then there exists an optimum solution $(H, w)$ such that the hypergraph $H$ is uniform and there exists a polynomial-time algorithm to find such an optimum solution. 
\end{theorem}
\begin{proof}
    Let $(G=(V, E), c:E\rightarrow \Z_+)$ be the input hypergraph and $r:\binom{V}{2}\rightarrow \Z_{\ge 0}$ be the input target connectivity function. 
    We consider the set function $R: 2^V\rightarrow \Z_{\ge 0}$ defined by $R(X)\coloneqq \max\{r(\{u, v\}): u\in X, v\in V'\setminus X\}$ for every non-empty proper subset $X\subseteq V$, $R(\emptyset)\coloneqq 0$, and $R(V)\coloneqq 0$. 
    %The function $R$ is symmetric skew-supermodular \knote{need to prove}. 
    Next, we consider the function $p: 2^V\rightarrow \Z$ defined by $p(X)\coloneqq R(X)-d_{(G, c)}(X)$ for every $X\subseteq V$. The function $p$ is known to be symmetric skew-supermodular (e.g., see \Cref{lemma:helper-for-p-max-oracle}). 
    %and there exists a strongly polynomial-time algorithm to implement \functionMaximizationOracle{p} \knote{need to prove}. 
    We note that a hypergraph $(H=(V, E_H), w:E_H\rightarrow \Z_+)$ is a feasible solution for the problem if and only if the hypergraph $(H, w)$ strongly covers the function $p$. Moreover, for a hypergraph $(H, w)$, its weighted size is equal to the sum of degree of vertices, i.e., $\sum_{e\in E_H}|e|w(e)=\sum_{u\in V}b_{(H, w)}(u)$. Hence, the goal is to find a hypergraph $(H, w)$ that strongly covers the function $p$ and has the minimum sum of degree of vertices. 
    Let $m \in \Z_{\ge 0}^V$ be a vector with minimum $\sum_{u\in V}m(u)$ such that $m(X)\ge p(X)$ for every $X\subseteq V$. 
    Then, $m(u)\le K_p$ for every $u\in V$ (otherwise, reducing $m(u)$ preserves feasibility and improves $\sum_{u\in V} m(u)$, a contradiction). 
    By \Cref{coro:StrongCoverViaUniformHypergraph:main} applied to the symmetric skew-supermodular function $p$ and the non-negative function $m$, there exists a near-uniform hypergraph $(H=(V, E), w: E\rightarrow \Z_+)$ such that $(H, w)$ strongly covers the function $p$, $b_{(H, w)}(u)=m(u)$ for every $u\in V$, and $|E|=O(|V|)$. Hence, $(H, w)$ is an optimum solution. 
    
    There exists a strongly polynomial-time algorithm to implement \functionMaximizationOracle{p} (e.g., see \Cref{lemma:helper-for-p-max-oracle}). Moreover, a vector $m \in \Z_{\ge 0}^V$ with minimum $\sum_{u\in V}m(u)$ such that $m(X)\ge p(X)$ for every $X\subseteq V$ can be computed in strongly polynomial time given access to \functionMaximizationOracle{p} (e.g., see \Cref{lem:Frank:optimizing-over-contrapolymatroid-skew-supermodular-function}). Hence, by the algorithmic conclusion of \Cref{coro:StrongCoverViaUniformHypergraph:main}, an optimum solution $(H, w)$ can be found in strongly polynomial time. 
    %Existence of a \emph{near-uniform} hypergraph with $O(|V|)$ hyperedges as an optimal solution along with a strongly polynomial-time algorithm to find such a solution follows by applying \Cref{coro:StrongCoverViaUniformHypergraph:main} to the same symmetric skew-supermodular function $p$ and the degree requirement function $m$ defined above.
\end{proof}

We also address the \emph{simultaneous} hypergraph local connectivity augmentation using hyperedges of minimum total weighted size problem: the input is two hypergraphs $(G^i=(V, E_i), c^i: E_i\rightarrow \Z_+)$ for $i\in [2]$ and two target connectivity functions $r^i: \binom{V}{2}\rightarrow \Z_{\ge 0}$ for $i\in [2]$, where $\max\{r^1(\{u, v\})-\lambda_{(G^1,c^1)}(u, v): u, v\in V, u\neq v\}=\max\{r^2(\{u, v\})-\lambda_{(G^2,c^2)}(u, v): u, v\in V, u\neq v\}$. The goal is to find a hypergraph $(H=(V, E_H), w: E_H\rightarrow \Z_+)$ 
with minimum $\sum_{e\in E_H}|e|w(e)$ (i.e., minimum total weighted size), 
%of minimum total weighted size, i.e., minimize $\sum_{e\in E_H}w(e)$ 
such that $\lambda_{(G^i+H, c^i+w)}(u,v)\ge r^i(\{u, v\})$ for every distinct $u, v\in V$ and every $i\in [2]$. 
Bern\'{a}th and Kir\'{a}ly \cite{Bernath-Kiraly} showed that if $\max\{r^1(\{u, v\})-\lambda_{(G^1,c^1)}(u, v): u, v\in V, u\neq v\}\neq \max\{r^2(\{u, v\})-\lambda_{(G^2,c^2)}(u, v): u, v\in V, u\neq v\}$, then the problem is NP-hard, so we include this assumption in the problem definition. 
They also showed that there exists an optimal solution for this problem that is near-uniform. 
Our results imply that this problem can be solved in strongly polynomial time. 

\begin{theorem}\label{thm:simultaneous-local-connectivity-augmentation}
    Simultaneous hypergraph local connectivity augmentation  using hyperedges of minimum total weighted size problem admits an optimum solution $(H, w)$ such that $H$ is near-uniform and has $O(|V|^2)$ hyperedges, where $V$ is the vertex set of the input instance. Moreover, such an optimum solution can be found in strongly polynomial time. 
    
    %can be solved in strongly polynomial time. In particular, there exists a strongly polynomial-time algorithm to return an optimum solution $(H, w)$ such that $H$ is near-uniform. 
\end{theorem}
The proof of \Cref{thm:simultaneous-local-connectivity-augmentation} is identical to the proof of \Cref{thm:local-connectivity-augmentation} -- construct a pair of symmetric skew-supermodular function $p_1$ and $p_2$ using functions $q$ and $r$ respectively similar to the proof of \Cref{thm:local-connectivity-augmentation}, find a vector $m\in \Z^V_{\ge 0}$ with minimum $\sum_{u\in V} m(u)$ such that $m(X)\ge \max\{p_1(X), p_2(X)\}$ for every $X\subseteq V$, and apply \Cref{coro:StrongCoverTwoFunctionsViaUniformHypergraph:main} to the functions $p_1, p_2$ and $m$. We omit the details in the interests of brevity. 
